Adjusted quantile residual for generalized linear models

Generalized linear models are widely used in many areas of knowledge. As in other classes of regression models, it is desirable to perform diagnostic analysis in generalized linear models using residuals that are approximately standard normally distributed. Diagnostic analysis in this class of models are usually performed using the standardized Pearson residual or the standardized deviance residual. The former has skewed distribution and the latter has negative mean, specially when the variance of the response variable is high. In this work, we introduce the adjusted quantile residual for generalized linear models. Using Monte Carlo simulation techniques and two applications, we compare this residual with the standardized Pearson residual, the standardized deviance residual and two other residuals. Overall, the results suggest that the adjusted quantile residual is a better tool for diagnostic analysis in generalized linear models.

==> quant_glm <==
@article{anscombe,
 title={Contribution to the discussion of H. Hotelling’s paper},
 author={Anscombe, FJ},
 journal={Journal of the Royal Statistical Society},
volume={15},
number={2},
pages={229--230},
year={1953},
}


@article{abdo,
title={Influence of dyslipidemia and diabetes mellitus on chronic periodontal disease},
author={Abdo,  Almeida  and  Ribeiro, Fabiano and Juliane and Cirano and Casat and Zaffalon, Marcio  and Ribeiro, Fernanda Vieira and Giampaoli, Viviana and Viana Casarin, Renato Corr{\^e}a and Pimentel, Suzana Peres},
journal={Journal of periodontology},
volume={84},
number={10},
pages={1401--1408},
year={2013},
}



@article{akaike,
author={Akaike, Hirotugu},
title  ={A new look at the statistical model identification},
journal={IEEE Transactions on Automatic Control},
volume={19},
number={6},
pages ={716-723},
year={1974},
}

@article{anderson,
title={Asymptotic theory of certain" goodness of fit" criteria based on stochastic processes},
author={Anderson, Theodore W and Darling, Donald A},
journal={The annals of mathematical statistics},
volume={23},
pages={193--212},
year={1952},
publisher={JSTOR.}
}

@article{anholeto2014,
title={Adjusted Pearson residuals in beta regression models},
author={Anholeto, Tatiana and Sandoval, M{\^o}nica C and Botter, Denise A},
 journal={Journal of Statistical Computation and Simulation},
volume={84},
pages={999--1014},
year={2014},
publisher={Taylor \& Francis.}
}

@book{atkinson,
title={Plots, transformations, and regression: an introduction to graphical methods of diagnostic regression analysis},
author={Atkinson, Anthony Curtis},
edition = {},
publishe={Clarendon Press},
address={Oxford},
year={1985},
}

@misc{belsley,
  title={Recession Diagnostics},
  author={Belsley, David A and Kuh, Edwin and Welsch, Roy E},
  year={1980},
  publisher={John Wiley and Sons, New York}
}

@article{bic,
  title={Estimating the dimension of a model},
  author={Schwarz, Gideon and others},
  journal={The annals of statistics},
  volume={6},
  number={2},
  pages={461--464},
  year={1978},
  publisher={Institute of Mathematical Statistics}
}


@article{bortoluzzo2011,
  title={Estimating total claim size in the auto insurance industry: a comparison between tweedie and zero-adjusted inverse gaussian distribution},
  author={Bortoluzzo, Adriana Bruscato and Claro, Danny Pimentel and Caetano, Marco Antonio Leonel and Artes, Rinaldo},
  journal={BAR-Brazilian Administration Review},
  volume={8},
  number={1},
  pages={37--47},
  year={2011},
  publisher={SciELO Brasil.}
}

@article{cook2008,
  title={Regression analysis of proportions in finance with self selection},
  author={Cook, Douglas O and Kieschnick, Robert and McCullough, Bruce D},
  journal={Journal of empirical finance},
  volume={15},
  number={5},
  pages={860--867},
  year={2008},
  publisher={Elsevier.}
}


@article{cole1992,
  title={Smoothing reference centile curves: the LMS method and penalized likelihood},
  author={Cole, Timothy J and Green, Pamela J},
  journal={Statistics in medicine},
  volume={11},
  number={10},
  pages={1305--1319},
  year={1992},
  publisher={Wiley Online Library}
}


@article{cook1977,
  title={Detection of influential observation in linear regression},
  author={Cook, R Dennis},
  journal={Technometrics},
  volume={19},
  pages={15--18},
  year={1977},
  publisher={JSTOR}
}



@article{cook1982,
 title={Residuals and influence in regression},
author={Cook, R Dennis and Weisberg, Sanford},
journal={Chapman and Hall},
volume={19},
pages={15--18},
year={1982},
publisher={New York: Chapman and Hall}
}

@book{cordeiro,
title={Modelos lineares generalizados e Extens{\~o}es},
author={Cordeiro, Gauss Moutinho and Dem{\'e}trio, Clarice GB},
year={2008},
publisher={Recife: UFRPE}
}

@article{cordeiro2009,
  title={The distribution of Pearson residuals in generalized linear models},
  author={Cordeiro, Gauss M and Simas, Alexandre B},
  journal={Computational Statistics \& Data Analysis},
  volume={53},
  number={9},
  pages={3397--3411},
  year={2009},
  publisher={Elsevier}
}

@article{cordeiro2004pearson,
  title={On Pearson's residuals in generalized linear models},
  author={Cordeiro, Gauss M},
  journal={Statistics \& probability letters},
  volume={66},
  number={3},
  pages={213--219},
  year={2004},
  publisher={Elsevier}
}


@ONLINE{cvm,
author = {Pereira, Leonardo and Novaes, D. Ana and Dias, P. Luciana and others},
title = {Fundos de investimentos,},
year = {2014},
url = {http://www.investidor.gov.br}
}

@article{davison,
  title={Deviance residuals and normal scores plots},
  author={Davison, AC and Gigli, A},
  journal={Biometrika},
  volume={76},
  number={2},
  pages={211--221},
  year={1989},
  publisher={Biometrika Trust}
}

@phdthesis{dias,
title={Modelos assim{\'e}tricos in aficionados de zeros},
author={Dias, Mariana Ferreira},
school={Universidade de S{\~a}o Paulo},
year={2014},
type={Disserta{\c{c}}{\~a}o de Mestrado em Estat\'istica.}
}


@article{dunn,
  title={Randomized quantile residuals},
  author={Dunn, Peter K and Smyth, Gordon K},
  journal={Journal of Computational and Graphical Statistics},
  volume={5},
  number={3},
  pages={236--244},
  year={1996},
  publisher={Taylor \& Francis.}
}


@article{dunnseries,
  title={Series evaluation of Tweedie exponential dispersion model densities},
  author={Dunn, Peter K and Smyth, Gordon K},
  journal={Statistics and Computing},
  volume={15},
  number={4},
  pages={267--280},
  year={2005},
  publisher={Springer.}
}

@article{feng2017randomized,
  title={Randomized Quantile Residuals: an Omnibus Model Diagnostic Tool with Unified Reference Distribution},
  author={Feng, Cindy and Sadeghpour, Alireza and Li, Longhai},
  journal={arXiv preprint arXiv:1708.08527},
  year={2017}
}


@article{feuerverger,
  title={On some methods of analysis for weather experiments},
  author={Feuerverger, Andrey},
  journal={Biometrika},
  volume={66},
  number={3},
  pages={655--658},
  year={1979},
  publisher={Biometrika Trust.}
}


@phdthesis{ferreira2005,
  title={Uma Abordagem Cl{\'a}ssica e Bayesiana para o Modelo de Tweedie},
  author={Ferreira, Fl{\'a}via},
  year={2005},
 school={Departamento de  Estat{\'\i}stica da Universidade Federal de S{\~a}o Carlos},
type={Disserta{\c{c}}{\~a}o do Programa de P{\'o}s-Gradua{\c{c}}{\~a}o em Estat{\'\i}stica}
}


@phdthesis{ferreira2008,
  title={Modelos de previs{\~a}o de perdas para cr{\'e}dito massificado},
 author={Ferreira, Jefferson},
  school={Ibmec. S{\~a}o Paulo},
  year={2008},
  type={Disserta{\c{c}}{\~a}o de Mestrado}
}



@techreport{fonseca,
  title={An{\'a}lise do Desempenho Recente de Fundos de Investimento no Brasil]},
  author={Fonseca, Nelson and Bressan, Aureliano and Iquiapaza, Robert and Guerra, Jo{\~a}o and others},
  year={2007},
  institution={University Library of Munich, Germany}
}


@book{hardin2007generalized,
  title={Generalized linear models and extensions},
  author={Hardin, James William and Hilbe, Joseph M and Hilbe, Joseph},
  year={2007},
  publisher={Stata press}
}


@article{heller,
 title={The zero-adjusted inverse Gaussian distribution as a model for insurance claims},
 author={Heller, Gillian and Stasinopoulos, Mikis and Rigby, Bob and others},
 booktitle={Proceedings of the 21th International Workshop on Statistical Modelling},
 volume={226233},
 year={2006}
}


@article{hoff,
title={Second stage DEA: Comparison of approaches for modelling the DEA score},
 author={Hoff, Ayoe},
 journal={European Journal of Operational Research},
 volume={181},
 number={1},
 pages={425--435},
 year={2007},
 publisher={Elsevier}
}


@book{hosmer,
 title={Applied logistic regression},
 author={Hosmer Jr, David W and Lemeshow, Stanley},
 year={2004},
 publisher={John Wiley \& Sons}
}


@article{hosmer1997,
 title={A comparison of goodness-of-fit tests for the logistic regression model},
 author={Hosmer, David W and Hosmer, Trina and Le Cessie, Saskia and Lemeshow, Stanley and others},
 journal={Statistics in medicine},
 volume={16},
 number={9},
 pages={965--980},
 year={1997}
}


@article{hosmer1991,
 title={The importance of assessing the fit of logistic regression models: a case study.},
 author={Hosmer, David W and Taber, Scott and Lemeshow, Stanley},
 journal={American journal of public health},
 volume={81},
 number={12},
 pages={1630--1635},
 year={1991},
 publisher={American Public Health Association}
}

@book{jorgensenb,
 title={The theory of dispersion models},
 author={Jorgensen, Bent},
volume={1},
 year={1997},
 publisher={Chapman and Hall/CRC}
}

@book{jong,
title={Generalized linear models for insurance data},
author={De Jong, Piet and Heller, Gillian Z and others},
volume={136},
year={2008},
 publisher={Cambridge University Press Cambridge}
}

@book{johnson,
title={Continuous univariate distributions},
author={Johnson, Norman L and Kotz, Samuel and Balakrishnan, Narayanaswamy},
year={1994},
volume={1-2},
publisher={New York: John Wiley \& Sons}
}


@article{jorgensen,
 title={Fitting Tweedie's compound Poisson model to insurance claims data},
 author={J{\o}rgensen, Bent and Paes De Souza, Marta C},
 journal={Scandinavian Actuarial Journal},
 volume={1994},
 number={1},
 pages={69--93},
 year={1994},
 publisher={Taylor \& Francis}
}

@article{klar2012specification,
  title={Specification tests for the response distribution in generalized linear models},
  author={Klar, Bernhard and Meintanis, Simos G},
  journal={Computational Statistics},
  volume={27},
  number={2},
  pages={251--267},
  year={2012},
  publisher={Springer}
}

@book{lawless,
  title={Statistical models and methods for lifetime data},
  author={Lawless, Jerald F},
  volume={362},
  year={2011},
  publisher={John Wiley \& Sons}
}

@book{liu2007,
title={On goodness-of-fit of logistic regression model},
author={Liu, Ying},
year={2007},
publisher={ProQuest}
}

@phdthesis{martinez,
 title={Modelos de regressao beta inflacionados},
author={Mart{\'i}nez, Raydonal Ospina},
year={2008},
 school={Universidade de S{\~a}o Paulo},
type={Tese de Doutorado em Estat\'istica.}
}

 @book{mccullagh,
  title={Generalized linear models},
  author={McCullagh, Peter and Nelder, John A},
  edition = {2},
  year={1989},
  publisher={CRC press}
}

@article{mccullagh1985,
  title={On the asymptotic distribution of Pearson's statistic in linear exponential-family models},
  author={McCullagh, Peter},
  journal={International Statistical Review/Revue Internationale de Statistique},
  pages={61--67},
  year={1985},
  publisher={JSTOR}
}



@article{nelder72,
  title={Generalized linear models},
  author={Nelder, J. A. and  Wedderburn, R. W. M.},
  journal={Journal of the Royal Statistical Society},
 volume={10},
  number={3},
 pages={370-384},
  year={1972}
}

@article{ospina,
  title={A general class of zero-or-one inflated beta regression models},
  author={Ospina, Raydonal and Ferrari, Silvia LP},
  journal={Computational Statistics \& Data Analysis},
  volume={56},
  number={6},
  pages={1609--1623},
  year={2012},
  publisher={Elsevier}
}

@phdthesis{ospina2008,
title={Modelos de regress{\~a}o beta inflacionados},
author={Ospina, R},
school={Instituto de Matem{\'a}tica e Estat{\'\i}stica da Universidade de S{\~a}o Paulo},
year={2008},
type={Tese do Programa de P{\'o}s-Gradua{\c{c}}{\~a}o em Estat{\'\i}stica}
}

@article{ospina2010,
title={Inflated beta distributions},
author={Ospina, Raydonal and Ferrari, Silvia LP},
 journal={Statistical Papers},
volume={51},
number={1},
pages={111--126},
year={2010},
 publisher={Springer}
}

@book{paula,
title={Modelos de regress{\~a}o: com apoio computacional},
author={Paula, Gilberto Alvarenga},
year={2013},
publisher={IME-USP S{\~a}o Paulo}
}

@article{pereira2012,
title={The truncated inflated beta distribution},
author={Pereira, Gustavo HA and Botter, Denise A and Sandoval, M{\^o}nica C},
 journal={Communications in Statistics-Theory and Methods},
 volume={41},
number={5},
pages={907--919},
year={2012},
publisher={Taylor \& Francis}
}

@article{pereira2017quantile,
  title={On quantile residuals in beta regression},
  author={Pereira, Gustavo H A},
  journal={Communications in Statistics-Simulation and Computation},
  volume  = {, in press},
  number  = {},
  pages   = {},
  year={2017}
}


@phdthesis{pereiratese,
 title={Modelos de regress{\~a}o beta inflacionados truncados},
author={de Araujo Pereira, Gustavo Henrique},
school={Instituto de Matem{\'a}tica e Estat{\'\i}stica da Universidade de S{\~a}o Paulo},
year={2012},
type={Tese do Programa de P{\'o}s-Gradua{\c{c}}{\~a}o em Estat{\'\i}stica}
}


@article{pereira,
title={A new residual in zero inflated regression models},
author={Pereira, Gustavo HA and Botter, Denise A and Sandoval, M{\^o}nica C},
journal={Proceedings of the 21th Simp\'osio Nacional de Probabilidade e Estat\'istica.},
 volume={""},
number={""},
pages={""},
year={2014}
}

@book{pace,
title={Principles of statistical inference: from a Neo-Fisherian perspective},
author={Pace, Luigi and Salvan, Alessandra},
volume={4},
year={1997},
publisher={World Scientific}
}


@article{pierce1986residuals,
  title={Residuals in generalized linear models},
  author={Pierce, Donald A and Schafer, Daniel W},
  journal={Journal of the American Statistical Association},
  volume={81},
  number={396},
  pages={977--986},
  year={1986},
  publisher={Taylor \& Francis Group}
}



@phdthesis{pousinho,
title={Pagamentos de sinistros},
author={Pousinho, Andr{\'e} Pereira},
year={2013},
school={Instituto Superior de Economia e Gest{\~a}o},
type={Disserta{\c{c}}{\~a}o de mestrado do  Instituto Superior de Economia e Gest{\~a}o}
}



@article{royston,
  title={The use of cusums and other techniques in modelling continuous covariates in logistic regression},
  author={Royston, Patrick},
  journal={Statistics in medicine},
  volume={11},
  number={8},
  pages={1115--1129},
  year={1992},
  publisher={Wiley Online Library}
}


@article{resti,
  title={Estimation of claim cost data using zero adjusted gamma and inverse Gaussian regression models},
  author={Resti, Yuliai and Ismail, Noriszura  and Jamaan, Saiful Hafizah },
  journal={Journal of Mathematics and Statistics},
 volume={9},
  number={3},
  pages={186-192},
  year={2013}
}

@article{rigby2005,
  title={Generalized additive models for location, scale and shape},
  author={Rigby, Robert A and Stasinopoulos, D Mikis},
  journal={Journal of the Royal Statistical Society: Series C (Applied Statistics)},
  volume={54},
  number={3},
  pages={507--554},
  year={2005},
  publisher={Wiley Online Library}
}

@book{rigby2015,
 title={Flexible Regression and Smoothing: Using GAMLSS in R},
 author={Stasinopoulos, D Mikis and Rigby, Robert A and Voudouris, Vlasios and Heller, Gillian and De Bastiani, Fernanda    },
 year={2017},
 publisher={Taylor \& Francis}
}

@incollection{rigby1996,
  title={Mean and dispersion additive models},
  author={Rigby, Robert A and Stasinopoulos, Mikis D},
  booktitle={Statistical theory and computational aspects of smoothing},
  pages={215--230},
  year={1996},
  publisher={Springer}
}


@article{rocha,
title={Mycoflora and co-occurrence of fumonisins and aflatoxins in freshly harvested corn in different regions of Brazil},
author={Rocha, Liliana O and Nakai, Viviane K and Braghini, Raquel and Reis, Tatiana A and Kobashigawa, Estela and Corr{\^e}a, Benedito},
journal={International journal of molecular sciences},
volume={10},
number={11},
 pages={5090--5103},
year={2009},
publisher={Molecular Diversity Preservation International}
}

@article{gamlss2016,
  title={Package gamlss. data},
  author={Stasinopoulos, Mikis and Rigby, Bob and Stasinopoulos, Maintainer Mikis},
  year={2016}
}

@article{simas2009,
  title={Adjusted Pearson residuals in exponential family nonlinear models},
  author={Simas, Alexandre B and Cordeiro, Gauss M},
  journal={Journal of Statistical Computation and Simulation},
  volume={79},
  number={4},
  pages={411--425},
  year={2009},
  publisher={Taylor \& Francis}
}

@article{stukel88,
 title={Generalized logistic models},
author={Stukel, Th{\'e}r{\`e}se A},
journal={Journal of the American Statistical Association},
volume={83},
 number={402},
pages={426--431},
year={1988},
publisher={Taylor \& Francis}
}

@article{stan,
  title={Generalized additive models for location scale and shape (GAMLSS) in R},
  author={Stasinopoulos, D Mikis and Rigby, Robert A},
  journal={Journal of Statistical Software},
  volume={23},
  number={7},
  pages={1--46},
  year={2007}
}

@misc{stasinopoulos08,
title={Instructions on how to use the GAMLSS package in R, 2008},
author={Stasinopoulos, DM and Rigby, B and Akantziliotou, C},
year={2014}
}

@article{stein,
  title={Linear models with an inverse gaussian poisson error distribution},
  author={Stein, Gillian Z and Juritz, June M},
  journal={Communications in Statistics-Theory and Methods},
  volume={17},
  number={2},
  pages={557--571},
  year={1988},
  publisher={Taylor \& Francis}
}

@article{tong,
  title={A zero-adjusted gamma model for mortgage loan loss given default},
  author={Tong, Edward NC and Mues, Christophe and Thomas, Lyn},
  journal={International Journal of Forecasting},
  volume={29},
  number={4},
  pages={548--562},
  year={2013},
  publisher={Elsevier}
}



@phdthesis{troiani,
  title={Aplicai{\c{c}}ao do modelo ZAIG (Zero Adjusted Inverse Gaussian) na an{\'{a}}lise de cart{\~{o}}es de cr{\'{e}}ditos},
  author={Troiani, Rafae Rodrigues},
 year={2009},
  school={ Faculdade Ibmec S{\~a}o Paulo},
  type={ Disserta{\c{c}}{\~a}o de Mestrado Profissional em Economia.}
}

@article{urbano2012wald,
  title={On Wald Residuals in Generalized Linear Models},
  author={Urbano, Mariana Ragassi and Borges Dem{\'e}trio, Clarice Garcia and Cordeiro, Gauss Moutinho},
  journal={Communications in Statistics-Theory and Methods},
  volume={41},
  number={4},
  pages={741--758},
  year={2012},
  publisher={Taylor \& Francis}
}


@article{venezuela,
  title={Estimating equations and diagnostic techniques applied to zero-inflated models for panel data},
  author={Venezuela, Maria Kelly and Artes, Rinaldo and others},
  journal={Electronic Journal of Statistics},
  volume={8},
  number={1},
  pages={1641--1660},
  year={2014},
  publisher={Institute of Mathematical Statistics}
}




@article{williams,
  title={Generalized linear model diagnostics using the deviance and single case deletions},
  author={Williams, DA},
  journal={Applied Statistics},
  pages={181--191},
  year={1987},
  publisher={JSTOR}
}




